Right Nilpotency of Braces of Cardinality $p^4$

We determine right nilpotency of braces of cardinality $p^4$. If a brace of cardinality $p^4$ has an abelian multiplicative group, then it is left and right nilpotent, so we only consider braces with non-abelian multiplicative groups. We show right nilpotency in all cases using the sufficient condition of $A\ast c=0$ for some central element $c$ of a brace $A$.

==> cp3cp32.tex <==

\section{$C_p\times C_{p^3}$}

In this document we try to characterise braces of cardinality $p^4$ with additive group $C_p\times C_{p^3}$.

Suppose the brace $(A,+,\circ)$ has $(A,+)\cong C_p\times C_{p^3}$. If a brace of cardinality $p^4$ has an abelian multiplicative group, then it is left and right nilpotent, so we will only consider braces with non-abelian multiplicative groups. A result of Bachiller's \cite[Theorem 2.5]{bachiller2016counterexample} states that for a group of order $p^n$ for $p>5$ with abelian additive group, the orders of elements in the additive and multiplicative groups of the brace coincide. This means that $(A,\circ)$ has an element of order $p^3.$ Now, \cite[point 65., page 86]{burnside1911theory} implies that the only non-abelian group of order $p^4$ with an element of order $p^3$ is defined by the relations
\[P^{p^3}=1, Q^p=1, Q^{-1}\circ P\circ Q = P^{1+p^2}.\]

We will call this group $G$. We have
\[(P^{1+p^2})^p = P^p\circ P^{p^3}=P^p.\]
Hence
\[P^p=Q^{-1}\circ P^p\circ Q.\]



Now \cite[Proposition 8]{rump2007braces} implies that $A^5=0$.


Lemma 4.4 from \cite{puljic2021braces} holds for our case as well. The lemma implies that \[P^{np^2}\in A^2 \text{ and } P^{np^2}\ast A^i \subseteq A^{i+2}.\]

We now derive a couple of identities we will use.

\begin{prop}
Let $B$ be a brace, $k,l\in\Z$ and $a,c\in B$. Then we have
\[c^k\ast(c^l\ast a)=c^l\ast(c^k\ast a).\]

\end{prop}

\begin{proof}
The proposition is proven using $c^k\circ c^d = c^d\circ c^k$ and $(a\circ b)\ast c = a\ast c +b\ast c + a\ast(b\ast c)$.
\end{proof}

\begin{prop}
We have $P^p\ast Q = Q\ast P^p$.
\end{prop}

\begin{proof}
We have $P^n\circ Q = Q\circ P^{n+np^2}$ which implies $P^n\ast Q + P^n = Q\ast P^{n+np^2}+P^{n+np^2}$.
In case of $n=p$ the result follows.

\end{proof}


\begin{lemma}
We have  $P^p\ast Q^c = Q^c\ast P^p$ for $c\in \Z$.
\end{lemma}

\begin{proof}

We have 
\begin{align*}
P^n\circ Q^c &= P^n\circ Q\circ Q^{c-1} = Q\circ P^{n+np^2}\circ Q\circ Q^{c-2}\\
&=Q^2\circ P^{n(1+p^2)^2}\circ Q^{c-2}\\
&= ... = Q^c\circ P^{(1+p^2)^cn}.
\end{align*}
Hence, for $n=p$, the statement follows.
\end{proof}

\begin{prop}\label{rel1}
We have
\[P^n\ast Q^c = Q^c\ast P^{(1+cp^2)n}+P^{(1+cp^2)n}-P^n. \]
\end{prop}

\begin{proof}
Use binomial theorem and the fact that $P^{p^l}=0$ for $l>2$.
\end{proof}


We can get the express the reverse relation as well.

\begin{cor}\label{QP}
Let $c,k\in\Z$. Then $Q^c\ast P^k = P^{k(1-cp^2)}\ast Q^c-P^k+P^{k(1-cp^2)}$.
\end{cor}

\begin{proof}
Consider Proposition \ref{rel1} and let $k=(1+cp^2)n$. Then $x=1-cp^2$ is such that $P^{xk}=P^n$. The relation follows.
\end{proof}

\begin{prop}\label{rel2}
Let $n,c\in\Z$ and $D\in A$. We have the following:
\[P^n\ast (Q^c\ast D)+P^n\ast D = Q^c\ast(P^{(1+cp^2)n}\ast D)+P^{(1+cp^2)n}\ast D,\]
\[P^p\ast(Q^c\ast D) = Q^c\ast(P^p\ast D).\]
\end{prop}

\begin{proof}
Consider $(P^n\circ Q^c)\ast D = (Q^c\circ P^{(1+cp^2)n})\ast D$.
\end{proof}


\begin{prop}
$P^p\in Z(A)$.
\end{prop}

\begin{proof}
Notice that as $P\circ Q = P^{1+p^2}\circ Q$, we can write any $a\in A$ as $a = Q^c\circ P^d$ for some $c,d\in \Z$. It follows that 
\[a\ast P^p = (Q^c\ast P^d+Q^c+P^d)\ast P^p = Q^c\ast P^p +P^p\ast P^d +Q^c\ast(P^p\ast P^d).\]
Now consider $P^p\ast a$. We have
\[P^p\ast a = P^p\ast (Q^c\ast P^d+Q^c+P^d) = P^p\ast(Q^c\ast P^d)+P^p\ast P^d+P^p\ast Q^c.\]
Now Proposition \ref{rel2} gives the result.
\end{proof}

\begin{prop}
Let $a=Q^c\circ P^d$ for some $c,d\in \Z$. Then we have
\begin{equation}
\begin{split}
    P^n \ast a= a\ast P^n &+ Q^c\ast (P^{ncp^2}\ast P^d) + P^n\ast (P^{ncp^2}\ast P^d)+P^{ncp^2}\ast P^d\\
    &+ Q^c\ast (P^n\ast P^{ncp^2})+Q^c\ast P^{ncp^2}+P^n\ast P^{ncp^2}.    
\end{split}
\end{equation}
In particular, if $n=kp^2$, we have
\[P^{kp^2}\ast a = a\ast P^{kp^2}.\]
\end{prop}

\begin{proof}
By calculation.
\end{proof}



Now, by \cite{puljic2021braces} if $c\in Z(A)$ is such that $A\ast c=0$, then $c\ast A=0$. Therefore $c$ generates an ideal $I$ in $A$ such that $I\ast A = A\ast I=0$. By a result of Bachiller's \cite{bachiller2016counterexample}, this implies that $A/I$ is right nilpotent, so $A$ is right nilpotent.

Therefore it suffices to show that $A\ast P^{p^2}=0$, as then $A$ is right nilpotent. Notice now that $P^{p^2}\in p^2 A$, so it suffices to prove that $A\ast p^2 A = 0$. As any element of $A$ is a product of $P$s and $Q$s, it suffices to prove $Q\ast p^2 A=0$ and $P\ast p^2 A = 0.$

We are going to prove these claims in $2$ separate cases. We start with the first case.

\subsection*{First Case}

\textbf{Notation.} We note that when we write $na\ast b$ for $n\in \Z$ and $a,b\in A$ it is implied that we mean $n(a\ast b)$.

We assume that there exist $x,y,x',y' \in \Z$ such that 
\[P\ast P = xP+yQ, \quad P\ast Q = x'P+y'Q.\]

Notice that as $pQ = 0$, we have $P\ast pP= pxP+pyQ = pxP.$ Hence $P\ast(P\ast(P\ast (P\ast pP)))=px^4 P=0,$ so \[p\mid x.\]

Further, $P\ast pQ = 0$ so $px'P=0$ and therefore \[p^2\mid x'.\]


\begin{prop}
$P\ast Q=x' P $ and $p\mid y.$
\end{prop}

\begin{proof}
We have 

\begin{align*}
    P\ast(P\ast Q) &= x' (P\ast P) + y'(P\ast Q)\\
    &= y'(P\ast Q).
\end{align*}
It follows that $P\ast(P\ast(P\ast(P\ast Q))) = y'^3 (P\ast Q)=0.$ Hence $p\mid y'$ and $P\ast Q= x'P.$

\end{proof}

\begin{cor}
$P\ast(P\ast Q)=0$ and $P\ast(P\ast(P\ast P))=0.$
\end{cor}

\begin{prop}\label{propPPn}
$P\ast P^n = \frac{1}{2}n(n-1) P\ast(P\ast P)+n(P\ast P).$
\end{prop}
\begin{proof}
We prove the proposition by induction. The base case clearly holds. Now, we have
\begin{align*}
    P\ast P^{n+1}&=P\ast(P\circ P^n) = P\ast (P\ast P^n)+P\ast P + P\ast P^n\\
    &=n(P\ast (P\ast P)) + P\ast P + \frac{1}{2}n(n-1) P\ast(P\ast P)+n(P\ast P)\\
    &=\frac{1}{2}n(n+1) P\ast(P\ast P)+(n+1)(P\ast P).
\end{align*}

\end{proof}


\begin{prop}
$P\ast Q^n = (n-1)P\ast(P\ast(Q\ast Q))+P\ast(Q\ast Q)+nx'P.$
\end{prop}
\begin{proof}
We prove the proposition by induction. The base case clearly holds. Now, we have
\begin{align*}
    P\ast Q^{n+1}&=P\ast(Q\circ Q^n) = P\ast (Q\ast Q^n)+P\ast Q + P\ast Q^n\\
    &=P\ast(P\ast (Q\ast Q))+nx'P\ast P + P\ast Q  \\
    &+ (n-1)P\ast(P\ast(Q\ast Q))+P\ast(Q\ast Q)+nx'P\\
    &=n(P\ast(P\ast(Q\ast Q)))+P\ast(Q\ast Q)+(n+1)x'P.
\end{align*}

\end{proof}


\begin{prop}\label{PkQn}
$P^k\ast Q^n=\frac{1}{2}k(2n-5+k)P\ast(P\ast(Q\ast Q))+kP\ast(Q\ast Q)+knx'P.$
\end{prop}
\begin{proof}
We prove the proposition by induction on k. The base case clearly holds. Now, we have
\begin{align*}
    P^{k+1}\ast Q^{n}&=(P\circ P^{k})\ast Q^n = P\ast (P^k\ast Q^n )+P\ast Q^n+ P^k\ast Q^n\\
    &= kP\ast (P\ast(Q\ast Q))+knx'P\ast P+P\ast Q\\
    &+\frac{1}{2}k(2n-5+k)P\ast(P\ast(Q\ast Q))+kP\ast(Q\ast Q)+knx'P\\
    &=\frac{1}{2}(k+1)(2n-4+k)P\ast(P\ast(Q\ast Q))+(k+1)P\ast(Q\ast Q)+(k+1)nx'P.
\end{align*}
\end{proof}

\begin{prop}
Let $a\in A.$ Then $P\ast p^2 a = 0$.
\end{prop}

\begin{proof}
We let $a = Q^c\circ P^d$ for some $c,d\in \Z$. Then 
\[P\ast p^2 a = P\ast p^2 (Q^c\ast P^d)+P\ast p^2 P^d.\]
Now by Proposition \ref{propPPn},
\[P\ast p^2 P^d=p^2 (P\ast P^d) = 0.\]
We have 
\[P\ast p^2 (Q^c\ast P^d) = P\ast p^2 (P^{d-dcp^2}\ast Q^c),\]
by Corollary \ref{QP}. Further, by Proposition \ref{PkQn}
\begin{align*}
    P\ast p^2 (P^{d-dcp^2}\ast Q^c) =0.
\end{align*}
\end{proof}



\begin{prop}\label{QPn}
$Q\ast P^n = c_n Q\ast (P\ast (P\ast P))+ b_n Q\ast (P\ast P)+ n Q\ast P $ for some constants $c_n, b_n.$
\end{prop}
\begin{proof}
We prove the proposition by induction. The base case clearly holds. Now, we have
\begin{align*}
    Q\ast P^{n+1} &= Q\ast (P\circ P^n) = Q\ast (P\ast P^n)+Q\ast P +Q\ast P^n\\
    &= \frac{1}{2}n(n-1) Q\ast (P\ast(P\ast P))+nQ\ast (P\ast P)+ Q\ast P\\
    &+c_n Q\ast (P\ast (P\ast P))+ b_n Q\ast (P\ast P)+ n Q\ast P\\
    &=c_{n+1} Q\ast (P\ast (P\ast P))+ b_{n+1} Q\ast (P\ast P)+ (n+1) Q\ast P.
\end{align*}
\end{proof}


\begin{prop}
Let $a\in A.$ Then $Q\ast p^2 a = 0$.
\end{prop}

\begin{proof}
We let $a = Q^c\circ P^d$ for some $c,d\in \Z$. Then by Corollary \ref{QP} and Proposition \ref{QPn} we have
\begin{align*}
    Q\ast p^2 a &= Q\ast p^2 (Q^c\ast P^d)+Q\ast p^2 P^d\\
    &=-Q\ast p^2 P^d+Q\ast p^2 P^{d-dcp^2}+Q\ast p^2 P^d\\
    &=p^2(c_{d-dcp^2} Q\ast (P\ast (P\ast P))+ b_{d-dcp^2} Q\ast (P\ast P)+ (d-dcp^2) Q\ast P)\\
    &=0,
\end{align*}
as $P\ast p^2 P=Q\ast p^2 P=0.$

\end{proof}

\subsection*{Second Case}
If there exist no  $x,y,x',y'\in \Z$ such that $P\ast P = xP+yQ, \quad P\ast Q = x'P+y'Q$, then there exists $x\in \Z$ such that 
\[Q=xP.\]

Note that $pQ = pxP=0$, which implies that 
\[p^2\mid x.\]

\begin{prop}
Let $a\in A$. Then $Q\ast p^2 a=0.$
\end{prop}

\begin{proof}
We let $a = P^n\circ Q^c$ for some $n,c\in \Z$. Note that 
\[p^2 a = p^2(P^n\circ Q^c) = P^n\circ p^2 Q^c + (p^2-1)P^n = p^2 P^n, \]
where we used the identity $a\circ nb=n(a\circ b)-(n-1)a.$
Therefore
\begin{align*}
    Q\ast p^2 a &= Q\ast p^2 P^n = p^2(Q\ast P)\\
    &=p^2 (P^{n-np^2}\ast Q-P^n+P^{n-np^2})\\
    &=-p^2P^n+p^2P^{n-np^2}\\
    &=0.
\end{align*}
\end{proof}


\begin{prop}\label{PPn}
$P\ast P^n = \frac{1}{6}(n-2)(n-1)n P\ast (P\ast (P\ast P))+ \frac{1}{2}n(n-1) P\ast (P\ast P)+ n (P\ast P).$
\end{prop}
\begin{proof}
We prove the proposition by induction. The base case clearly holds. Now, we have
\begin{align*}
    P\ast P^{n+1} &= P\ast (P\circ P^n) = P\ast (P\ast P^n)+P\ast P +P\ast P^n\\
    &= \frac{1}{2}n(n-1)P\ast( P\ast (P\ast P))+ n P\ast(P\ast P)+P\ast P\\
    &+\frac{1}{6}(n-2)(n-1)n P\ast (P\ast (P\ast P))+ \frac{1}{2}n(n-1) P\ast (P\ast P)+ n( P\ast P)\\
    &=\frac{1}{6}(n-1)n(n+1) P\ast (P\ast (P\ast P))+ \frac{1}{2}n(n+1) P\ast (P\ast P)+ (n+1) P\ast P.
\end{align*}
\end{proof}

\begin{prop}
$p^2(P\ast P)\in A^3$ and $P\ast P^{p^2} = \frac{1}{2}p^2(p^2-1) P\ast (P\ast P)+ p^2 (P\ast P).$
\end{prop}

\begin{proof}
By Proposition \ref{PPn} we have
\[P\ast P^{p^2} =\frac{1}{6}(p^2-2)(p^2-1)p^2 P\ast (P\ast (P\ast P))+ \frac{1}{2}p^2(p^2-1) P\ast (P\ast P)+ p^2 (P\ast P), \]
which implies that $p^2(P\ast P)\in A^3. $ This in turn implies that 
\[P\ast P^{p^2} = \frac{1}{2}p^2(p^2-1) P\ast (P\ast P)+ p^2 (P\ast P). \]
\end{proof}

\begin{cor}
$p^2 P\ast(P\ast P) = P\ast(P\ast P^{p^2}).$
\end{cor}

\begin{prop}
$p^2 P\ast(P\ast P^n)=np^2 P\ast (P\ast P)=0$ for all $n\in\Z$ and $P^{p^2} = p^2 P$.
\end{prop}
\begin{proof}
As before we have
\[P\ast P^n =  \frac{1}{2}n(n-1) P\ast (P\ast P)+ n (P\ast P),\]
which implies
\[p^2 P\ast(P\ast P^n)=np^2 P\ast (P\ast P).\]

Recall that $P^{p^2}\in p^2 A.$ Let $d\in A$. Then we can write $d = P^{d_1}\circ Q^{d_2}$ and $P^{p^2}=p^2 d=p^2 P^{d_1}.$
We have
\begin{align*}
    p^2 P\ast (P\ast P) = p^2 P\ast (P\ast P^{d_1}) = p^2 d_1 P\ast(P\ast P).
\end{align*}
This implies $d_1=1$ and $P^{p^2} = p^2 P$.

We have
\[P\ast P^{p^2} =  \frac{1}{2}p^2(p^2-1) P\ast (P\ast P)+ p^2 (P\ast P),\]
so
\[\frac{1}{2}p^2(p^2-1) P\ast (P\ast P)=0.\]
As $\frac{1}{2}(p^2-1)$ is an integer which is not divisible by $p$, it follows that $p^2P\ast (P\ast P)=0.$
\end{proof}


\begin{cor}\label{np2pp}
$p^2(P\ast P^n) = np^2(P\ast P).$
\end{cor}

\begin{prop}
$p^2P^{-1}=-p^2 P.$
\end{prop}

Recall that $P^{p^2}, P^{-p^2}\in p^2 A$, so we can write $P^{p^2}=p^2 b$, $P^{-p^2}=p^2 c$ for some $b,c\in A$. Let $b=P^{b_1}\circ Q^{b_2}, c=P^{c_1}\circ Q^{c_2}$, so \[P^{p^2}=p^2 P^{b_1}, \quad P^{-p^2}=p^2 P^{c_1}.\] Note that $p\nmid b_1, c_1.$
Now consider $P^{-p^2}\ast P^{p^2}$. We have
\begin{align*}
    P^{-p^2}\ast P^{p^2} &= -P^{-p^2}-P^{p^2}\\
    &=-p^2P^{c_1}-p^2P^{b_1}.
\end{align*}
Also, as $P^{kp^2}\in Z(A)$
\begin{align*}
    P^{-p^2}\ast P^{p^2} &= p^2(P^{-p^2}\ast P^{b_1})\\
    &=p^2(P^{b_1}\ast p^2P^{c_1})\\
    &=0,
\end{align*}
so $p^2 P^{b_1}=-p^2P^{c_1}$.

Therefore
\begin{align*}
    P^{-p^2}\ast P^{p^2} &=-(p^2P^{b_1}\ast p^2P^{b_1})\\
    &=-(p^2 P^{b_1})^2+2p^2P^{b_1}\\
    &=0,
\end{align*}
so $(p^2 P^{b_1})^2=2p^2P^{b_1}$, which implies $(p^2 P^{b_1})^n=np^2P^{b_1}$. Hence $(P^{p^2})^n=nP^{p^2}$ and similarly $(P^{-p^2})^n=nP^{-p^2}$. It follows that $P\ast P^{-p^2} = P\ast -P^{p^2}=-p^2(P\ast P).$



Now we have
\begin{align*}
    P\ast P^{-p^2} &= P\ast (-p^2 P^{b_1})\\
    &=-p^2(P\ast P^{b_1})\\
    &=-p^2 b_1 (P\ast P)
\end{align*}
by Corollary \ref{np2pp}. Hence $b_1=1.$ Now we have
\begin{align*}
    P\ast P^{-p^2} &= P\ast (p^2 P^{c_1})\\
    &=p^2(P\ast P^{c_1})\\
    &=p^2 c_1 (P\ast P),
\end{align*}
so $c_1=-1.$

\begin{cor}
Let $a\in A$. Then $P\ast p^2 a = 0.$
\end{cor}

\begin{proof}
We let $a = P^n\circ Q^c$ for some $n,c\in \Z$. Note that as before
\[p^2 a = p^2 P^n. \]
We have
\[P\ast p^2 P^n = np^2 P\ast P.\]
Consider $p^2(P\ast P^{p^2-1}).$ We have
\begin{align*}
    p^2(P\ast P^{p^2-1}) &= -p^2 (P\ast P)\\
    &= p^2(P\ast (P^{p^2}\circ P^{-1}))\\
    &= p^2(P\ast (P\ast P^{p^2})+P\ast P^{-1}+P\ast P^{p^2})\\
    &=-p^2 P-p^2P^{-1}\\
    &=0.
\end{align*}


\end{proof}

